Aligning Language Models with Preferences through f-divergence Minimization

Aligning language models with preferences can be posed as approximating a target distribution representing some desired behavior. Existing approaches differ both in the functional form of the target distribution and the algorithm used to approximate it. For instance, Reinforcement Learning from Human Feedback (RLHF) corresponds to minimizing a reverse KL from an implicit target distribution arising from a KL penalty in the objective. On the other hand, Generative Distributional Control (GDC) has an explicit target distribution and minimizes a forward KL from it using the Distributional Policy Gradient (DPG) algorithm. In this paper, we propose a new approach, f-DPG, which allows the use of any f-divergence to approximate any target distribution that can be evaluated. f-DPG unifies both frameworks (RLHF, GDC) and the approximation methods (DPG, RL with KL penalties). We show the practical benefits of various choices of divergence objectives and demonstrate that there is no universally optimal objective but that different divergences present different alignment and diversity trade-offs. We show that Jensen-Shannon divergence strikes a good balance between these objectives, and frequently outperforms forward KL divergence by a wide margin, leading to significant improvements over prior work. These distinguishing characteristics between divergences persist as the model size increases, highlighting the importance of selecting appropriate divergence objectives.

==> previous.appendices.formal.tex <==
\section{TMP-formal: temporary placeholder for displaced material}

\subsection{TMP-formal-table}
\begin{table*}
\begin{centering}
\begin{tabular}{ccccc}
\toprule
$D_f(\pit||p)$ & {\footnotesize{}$f$} & {\footnotesize{}$f'$} & {\footnotesize{}$f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)$}& {\footnotesize{}$f^{'}(\infty)$}\tabularnewline
\midrule
{\footnotesize{}forward KL} & {\footnotesize{}$f(t)=-\log t$} & {\footnotesize{}$f^{'}(t)=-\frac{1}{t}$} & {\footnotesize{}$-\frac{p(x)}{\pi_{\theta}(x)}$}& {\footnotesize{}$0$}\tabularnewline
% \hline 
{\footnotesize{}reverse KL} & {\footnotesize{}$f(t)=t\log t$} & {\footnotesize{}$f^{'}(t)=\log t+1$} & {\footnotesize{}$-\left(\log\frac{p(x)}{\pi_{\theta}(x)}\right)+1$}& {\footnotesize{}$\infty$}\tabularnewline
% \hline 
Total variation & {\footnotesize{}$f(t)=|1-t|$} & {\footnotesize{}$f^{'}(t)=\begin{cases}
1 & \text{for }t>1\\
-1 & \text{for }t<1
% \\\text{undefined} & \text{for }t=1
\end{cases}$} & {\footnotesize{}$\begin{cases}
1 & \text{for }\frac{\pi_{\theta}(x)}{p(x)}>1\\
-1 & \text{for }\frac{\pi_{\theta}(x)}{p(x)}<1
% \\\text{undefined} & \text{for }\pi_{\theta}(x)=p(x)
\end{cases}$}& {\footnotesize{}$1$}\tabularnewline
% \hline 
{\footnotesize{}Jensen-Shannon} & {\footnotesize{}$f(t)=t\log\frac{2t}{t+1}+\log\frac{2}{t+1}$} & {\footnotesize{}$f^{'}(t)=\log\frac{2t}{t+1}$} & {\footnotesize{}$\log 2-\log\left(1+\frac{p(x)}{\pi_{\theta}(x)}\right)$}& {\footnotesize{}$\log 2$}\tabularnewline
% \hline 
{\footnotesize{}Squared Hellinger distance} & {\footnotesize{}$f(t)=(1-\sqrt{t})^{2}$} & {\footnotesize{}$f^{'}(t)=1-\frac{1}{\sqrt{t}}$} & {\footnotesize{}$1-\sqrt{\frac{p(x)}{\pi_{\theta}(x)}}$}& {\footnotesize{}$1$}\tabularnewline
% \hline 
{\footnotesize{}Chi-squared divergence} & {\footnotesize{}$f(t)=(t-1)^{2}$} & {\footnotesize{}$f^{'}(t)=2(t-1)$} & {\footnotesize{}$2\left(\frac{\pi_{\theta}(x)}{p(x)}-1\right)$}& {\footnotesize{}$\infty$}\tabularnewline
% \hline 
{\footnotesize{}Le Cam distance} & {\footnotesize{}$f(t)=\frac{1-t}{2t+2}$} & {\footnotesize{}$f^{'}(t)=-\frac{1}{(1+t)^{2}}$} & {\footnotesize{}$-\left(\frac{p(x)}{p(x)+\pi_{\theta}(x)}\right)^{2}$}& {\footnotesize{}$0$}\tabularnewline
\bottomrule
\end{tabular}
\par\end{centering}
\caption{Some common $f$-divergences $D_f(\pi_\theta||p)$. 
%Note that forward KL divergence and reverse KL divergence  $D_f(p||\pi_\theta)$ instead of $D_f(\pi_\theta||p)$.
In the convention of this table, the $f$ shown corresponds to the order of arguments $D_f(\pit||p)$. Thus the forward KL between the target $p(x)$ and the model, $\text{KL}(p||\pit)$, corresponds to $D_{-\!\log t} (\pit||p)$, and similarly for the reverse KL, $\text{KL}(\pit||p)$, which corresponds to $D_{t \log t} (\pit||p)$, etc. Note that for symmetric divergences (TV and JS) the order of arguments is indifferent\ptmdI{: $\text{TV}(\pit||p)=\text{TV}(p||\pit)$, $\text{JS}(\pit||p)=\text{JS}(p||\pit)$.}
\label{tab:f-dpg-loss-appendix}}
\end{table*}

\subsection{TMP-formal-simplified-theorem}

\begin{thm*}[Theorem 1 repeated]
\label{thm:f-dpg-appendix}
Let $p$ and $\pit$ be distributions over a discrete set $\mathcal{X}$ such that  at least one of the following  conditions holds: 
(i) $\forall \theta \in \Theta, \Supp(p)\subset \Supp(\pit)$, or 
(ii) $\Supp(\pit)$ does not depend on $\theta$. Then:
% \ptmdI{$Supp(\pit)$ does not change with $\theta$,}
% $Supp(p) \subset Supp(\pit)$, 
% then:\fmdI{(13/01/2023) Note the change in the condition. I think this is more general, but can be discussed.}
%\fmdI{We should say somewhere something about $f'(\pit(x)/0$) in this equation.}
\begin{align}
    \nabla_{\theta}D_{f}(\pi_{\theta}||p)=E_{x\sim\pi_{\theta}}\left[f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)\nabla_{\theta}\log\pi_{\theta}(x)\right].
\label{Eq.:fdpg-gradient-appendix}
\end{align}
\end{thm*}
\ptmdI{The full proof of this theorem is provided in Appendix  \ref{app:proofs}, but let's already give a sketch, under the more restrictive assumption that $Supp(\pit)=Supp(p
) = S$.}
Based on Eq. \eqref{Eq.:f-divergence-simplified} we then have:\fmdI{(08/01/2023) This takes a lot of space. Should we delegate the whole proof (including the special case) to the Appendix?}
\fdyI{Hmm, I think that the straight forward proof for the special case is kind of attractive point that we have. For me, I would look for another section to save the space}
 % $D_{f}(\pi_{\theta}||p)=\sum_{\forall x}p(x)f\left(\frac{\pi_{\theta}(x)}{p(x)}\right).$
\begin{align*}
\nabt D_{f}(\pit||p) &= \nabt\ \ \E_{x\sim p}\ f(\frac{\pit(x)}{p(x)})\\
& =\nabt \sum_{x\in S}p(x)f\left(\frac{\pit(x)}{p(x)}\right)\\
 % & =\sum_{x\in S}p(x)\nabt f\left(\frac{\pit(x)}{p(x)}\right)\\
 & =\sum_{x\in S}p(x)f^{'}\left(\frac{\pit(x)}{p(x)}\right)\nabt \frac{\pit(x)}{p(x)}\\
 & =\sum_{x\in S}f^{'}\left(\frac{\pit(x)}{p(x)}\right)\nabt \ \pit(x)\\
 & =\sum_{x\in S}\pit(x)f^{'}\left(\frac{\pit(x)}{p(x)}\right)\nabt\log\pit(x)\\
 &= E_{x\sim\pit}\left[f^{'}\left(\frac{\pit(x)}{p(x)}\right)\nabt \log\pit(x)\right],
\end{align*}
where the third line involves an application of the chain-rule for the multidimensional variable $\theta$.

% \begin{proof}
% See Appendix \ref{app:proofs}
% \end{proof}
% In third equation we used chain rule, and the term $\nabla_{\theta}\frac{\pi_{\theta}(x)}{p(x)}$ makes the expectation with respect to $p(x)$ canceled out. The last equation we used log derivative trick, so that this can be approximated with samples from $\pi_{\theta}$. 

% \fmdI{(06/01/2023) I stopped my updating here, will continue later.}







\newpage
 
\section{$f$-divergences: equivalent definitions}\label{app:generalized_divergence}
Here we give a general definition of f-divergences between two probability distributions, without restrictions on the supports, in a useful ``symmetrical'' format, following \cite{liese2006divergences}. We then show that this definition is equivalent with the definition of Eq.~\ref{Eq.:f-divergence} \cite{polyanski},
\fmdI{(11/01/2023) I do not see this proof yet, will add it!}
\fdyI{I meant the general f-divergence can be simplfied to Eq. \ref{Eq.:f-divergence-simplified} (not Eq.~\ref{Eq.:f-divergence}) of which proof was intended in  Eq. ~\ref{Eq.:f-divergence-simplified2}}
and then
give examples of common $f$-divergences in the notation of the general definition.
\begin{definition*}[$f$-divergence: ``symmetrical'' format]
The $f$-divergence between two probability distributions $p$ and
$q$ over a discrete set $\mathcal{X}$ can be defined as
\begin{align}
D_{f}(p||q)\doteq \sum_{\{x:\ p(x)>0,\ q(x)>0\}}q(x)\ f(\frac{p(x)}{q(x)}) \quad +f(0)\ q(p=0) \quad +f^{*}(0)\ p(q=0)
\label{eq:generalized_divergence}
\end{align}


where the generator function $f:\ptmdI{(0,\infty)}\rightarrow\mathbb{R}$%
\fmdI{(11/01/2023) We need to use the open interval $(0,\infty)$ because $f$ need not be  defined in $0$ (e.g. $-\log t$), although it can be extended to $0$ with some care.}
is a convex function satisfying $f(1)=0$.
We denote by $q(p=0)$
the $q$-mass of the set $\{x:p(x)=0\}$, i.e. $q(p=0)=\sum_{\{x:p(x)=0\}}q(x)$
and similarly for $p(q=0)$.  
\end{definition*}
In this definition, the function $f^{*}(t)$ is the so-called \emph{perspective transform} of $f$
defined by $f^{*}(t)=t\ f(\frac{1}{t})$. It can be shown to also be a convex function
$f^{*}:\ptmdI{(0,\infty)} \rightarrow\mathbb{R}$ with $f^{*}(1)=0$ and
$f^{**}=f$. Also, $f(0) \in (0,\infty]$ can be defined as the (always existing) limit $f(0)\doteq \lim_{t\rightarrow 0} f(t)$, and similarly $f^{*}(0) \in (0,\infty]$ as $f^{*}(0)\doteq \lim_{t\rightarrow 0} f^{*}(t) = \lim_{t\rightarrow 0}\ t\ f(1/t)$ \cite{hiriart2013convex}. 



\ptmdI{HHHHH Here now (11/01/2023) HHHHH}






We now define the convention following \citet{liese2006divergences, polyanski}: 
\begin{itemize}
\item $f(0)=\lim_{t\rightarrow0}f(t)$, $f^{*}(0)=\lim_{t\rightarrow0}tf(\frac{1}{t})$
\item $0f(\frac{a}{0})=\lim_{t\rightarrow0}tf(\frac{a}{t})=af^{*}(0)$ for
$a>0$
\item $0f(0)=0,\ 0f^{*}(0)=0$, including the case where $f(0)=\infty$
\item $0f(\frac{0}{0})=0$
\end{itemize}
While it is not necessary for Theorem \ref{thm:f-dpg}, we show that, using the definition defined above, the general $f$-divergence without the assumption on the support can be simplified as follows.\label{Eq.:f-divergence-simplified2}
\begin{align*}
D_{f}(p||q) & =\sum_{\{x:p(x)>0,\ q(x)>0\}}q(x)f(\frac{p(x)}{q(x)})+f(0)q(p=0)+f^{*}(0)p(q=0)\\
 & =\sum_{\{x:p(x)q(x)>0\}}q(x)f(\frac{p(x)}{q(x)})+\sum_{\{x:p(x)=0,q(x)>0\}}q(x)f(0)+\sum_{\{x:p(x)>0,q(x)=0\}}q(x)f^{*}(0)+\sum_{\{x:p(x)=0,q(x)=0\}}0\\
 & =\sum_{\{x:p(x)q(x)>0\}}q(x)f(\frac{p(x)}{q(x)})+\sum_{\{x:p(x)=0,q(x)>0\}}q(x)f(\frac{p(x)}{q(x)})+\\ &\quad \sum_{\{x:p(x)>0,q(x)=0\}}q(x)f(\frac{p(x)}{q(x)})+\sum_{\{x:p(x)=0,q(x)=0\}}q(x)f(\frac{p(x)}{q(x)})\\
 & =\sum_{\forall x}q(x)f(\frac{p(x)}{q(x)})
\end{align*}


We now see how the generalized definition of $f$-divergence can be
adopted to the common divergences. 

\paragraph*{Forward, reverse KL}

\[
\text{KL}(p||q)=D_{f}(p||q)=D_{f^{*}}(q||p)
\]
 where $f(t)=t\log t$ with $f(0)=0,$$f^{*}(t)=-\log t$ with $f^{*}(0)=\infty$.
We can write $\text{KL}(p||q)$ with the generalized $f$-divergence;
\begin{align*}
\text{KL}(p||q) & =\sum_{\{x:p(x)>0,\ q(x)>0\}}q(x)f(\frac{p(x)}{q(x)})+f(0)q(p=0)+f^{*}(0)p(q=0)\\
 & =\sum_{\{x:p(x)>0,\ q(x)>0\}}q(x)\frac{p(x)}{q(x)}\log\frac{p(x)}{q(x)}+0+\infty p(q=0)\\
 & =\begin{cases}
\sum_{\{x:p(x)>0\}}p(x)\log\frac{p(x)}{q(x)} & \text{if }p(q=0)>0\\
\infty & \text{o.w.}
\end{cases}\\
 & =\begin{cases}
E_{x\sim p}\left[\log\frac{p(x)}{q(x)}\right] & \text{if }p(q=0)>0\\
\infty & \text{o.w.}
\end{cases}
\end{align*}
 

Similarly we have $\text{KL}(q||p)=\infty$ with $f(t)=t\log t$, we get 
\[
KL(q||p)=\begin{cases}
E_{x\sim q}\left[\log\frac{q(x)}{p(x)}\right] & \text{if }q(p=0)>0\\
\infty & \text{o.w.}
\end{cases}
\]


\paragraph*{Total variation divergence}

For Total variation divergence, 
\[
TV(p||q)=D_{f}(p||q)=D_{f^{*}}(q||p)=TV(q||p)
\]
with $f(t)=\frac{1}{2}|1-t|$ with $f(0)=\frac{1}{2}$ and $f^{*}(t)=f(t)$,
and $f^{*}(0)=\frac{1}{2}$. We can write $TV(p||q)$ with the generalized
$f$-divergence as follows
\begin{align*}
TV(p||q) & =\sum_{\{x:p(x)>0,\ q(x)>0\}}q(x)f(\frac{p(x)}{q(x)})+f(0)q(p=0)+f^{*}(0)p(q=0)\\
 & =\frac{1}{2}\sum_{\{x:p(x)>0,\ q(x)>0\}}q(x)\left|1-\frac{p(x)}{q(x)}\right|+\frac{1}{2}q(p=0)+\frac{1}{2}p(q=0)
\end{align*}
For example, in the extreme case where $\text{Supp}(p)\cap\text{Supp}(p)=\emptyset$,
we get the first term null, and second and third term equal to 0.5,
implying that $TV(p||q)=1$.
\section{Proofs and definitions}\label{app:proofs}

\begin{proof}[proof of Theorem \ref{thm:f-dpg}]
Note that without the restriction on the support of $p(x)$,
\[
D_{f}(\pi_{\theta}||p)=\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}p(x)f(\frac{\pi_{\theta}(x)}{p(x)})+f(0)p(\pi_{\theta}=0)+f^{*}(0)\pi_{\theta}(p=0)
\]
therefore, 
\begin{align*}
\nabla_{\theta}D_{f}(\pi_{\theta}||p) & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}p(x)\nabla_{\theta}f(\frac{\pi_{\theta}(x)}{p(x)})+f^{*}(0)\nabla_{\theta}\pi_{\theta}(p=0)+f(0)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}p(x)f^{'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\frac{\pi_{\theta}(x)}{p(x)}+f^{*}(0)\nabla_{\theta}\pi_{\theta}(p=0)+f(0)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}\pi_{\theta}(x)f^{'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)+f^{*}(0)\nabla_{\theta}\pi_{\theta}(p=0)+f(0)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}\pi_{\theta}(x)f^{'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)+f^{*}(0)\nabla_{\theta}\sum_{\{x:p(x)=0,\pi_{\theta}(x)>0\}}\pi_{\theta}(x)\\
 &\quad +f(0)\nabla_{\theta}p(\pi_{\theta}=0),\ \text{by definition of }\pi_{\theta}(p=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}\pi_{\theta}(x)f^{'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)+\sum_{\{x:p(x)=0,\pi_{\theta}(x)>0\}}\pi_{\theta}(x)f^{*}(0)\nabla_{\theta}\log\pi_{\theta}(x)\\
 &\quad +f(0)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}\pi_{\theta}(x)f^{'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)+\sum_{\{x:p(x)=0,\pi_{\theta}(x)>0\}}\pi_{\theta}(x)f^{'}(\infty)\nabla_{\theta}\log\pi_{\theta}(x)\\
 &\quad +f(0)\nabla_{\theta}p(\pi_{\theta}=0),\ \because f^{*}(0)=f^{'}(\infty)\\
 & =\sum_{\{x:\pi_{\theta}(x)>0\}}\pi_{\theta}(x)f^{'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)+f(0)\nabla_{\theta}p(\pi_{\theta}=0)
\end{align*}

The condition (i) stating that the support of $p$ is contained in the support of $\pi_{\theta}$ for all $\theta \in \Theta$ implies that $\nabla_{\theta}p(\pi_{\theta}=0)=\nabla_{\theta}0=0$, and the condition (ii) that the support of $\pi_{\theta}$ does not depend on $\theta$ further implies that $\nabla_{\theta}p(\pi_{\theta}=0)=0$, which concludes the proof.
% The condition (i) $\forall \theta \in \Theta, \Supp(p)\subset \Supp(\pit)$ implies that $\nabla_{\theta}p(\pi_{\theta}=0)=\nabla_{\theta}0=0$, and 
% (ii) $\Supp(\pit)$ does not depend on $\theta$ further implies $\nabla_{\theta}p(\pi_{\theta}=0)=0$, which
% concludes the proof.
\end{proof}

Especially, in the context of LMs, $\pi_{\theta}$ is typically a standard softmax-based autoregressive model which has full support over $\mathcal{X}$, meaning that $Supp(\pi_{\theta}) = \mathcal{X}$ and ${x:\pi_{\theta}(x)=0}=\emptyset$, thus satisfying condition (i).
% it is clear for all $x\in\mathcal{X}$, there
% exist $\delta>0\ \text{such that }\pi_{\theta}(x)>\delta$. 


Note that we use the notation $f^{'}(\infty)\doteq f^{*}(0)$ which is employed by \cite{polyanski} and is motivated by the fact that $\lim_{t\rightarrow\infty}f^{'}(t)=\lim_{t\rightarrow\infty}\frac{1}{t}f(t)=f^{*}(0)$ (See \citep{hiriart2013convex}). This notation allows to write $f^{'}(\frac{\pi_{\theta}(x)}{p(x)})$ instead of $f^{\ast}(0)$ when
$p(x)=0$ and $\pi_{\theta}(x)>0$ and therefore to simplify the writing
of $\nabla_{\theta}D_{f}(\pi_{\theta},p)$.

\begin{thm*}[Theorem \ref{thm:f-dpg} with $D_f(p||\pit)$]
Let $p$ and $\pit$ be distributions over a discrete set $\mathcal{X}$ such that at least one of the following  conditions holds: 
(i) $\forall \theta \in \Theta, \Supp(p)\subset \Supp(\pit)$, or 
(ii) $\Supp(\pit)$ does not depend on $\theta$.
Then:
\[
\nabla_{\theta}D_{f}(p||\pi_{\theta})=E_{x\sim\pi_{\theta}}\left[f^{*'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)\right]
\]
\end{thm*}

\begin{proof}
Note that without the restriction on the support of $p(x),$
\begin{align*}
D_{f}(p||\pi_{\theta}) & =\sum_{\{x:\pi_{\theta}(x)p(x)>0\}}\pi_{\theta}(x)f(\frac{p(x)}{\pi_{\theta}(x)})+f(0)\pi_{\theta}(p=0)+f^{*}(0)p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)p(x)\ge0\}}\pi_{\theta}(x)f(\frac{p(x)}{\pi_{\theta}(x)})+f^{*}(0)p(\pi_{\theta}=0)
\end{align*}
with $f(0)=f(\frac{p(x)}{\pi_{\theta}(x)})$ for $\{x:\pi_{\theta}(x)>0,p(x)=0\}$
and $f(0)\pi_{\theta}(p=0)=\sum_{\{x:\pi_{\theta}(x)>0,p(x)=0\}}\pi_{\theta}(x)f(\frac{p(x)}{\pi_{\theta}(x)})$.
Therefore, 
\begin{align*}
\nabla_{\theta}D_{f}(p||\pi_{\theta}) & =\sum_{\{x:\pi_{\theta}(x)>0,p(x)\ge0\}}\nabla_{\theta}\pi_{\theta}(x)f(\frac{p(x)}{\pi_{\theta}(x)})+\sum_{\{x:\pi_{\theta}(x)p(x)\ge0\}}\pi_{\theta}(x)f^{'}(\frac{p(x)}{\pi_{\theta}(x)})(-\frac{p(x)}{\pi_{\theta}(x)^{2}})\nabla_{\theta}\pi_{\theta}(x)\\&\qquad+f^{'}(\infty)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)>0,p(x)\ge0\}}\nabla_{\theta}\pi_{\theta}(x)\left[f(\frac{p(x)}{\pi_{\theta}(x)})-f^{'}(\frac{p(x)}{\pi_{\theta}(x)})(\frac{p(x)}{\pi_{\theta}(x)})\right]+f{}^{'}(\infty)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)>0,p(x)\ge0\}}\nabla_{\theta}\pi_{\theta}(x)\left[\frac{p(x)}{\pi_{\theta}(x)}f^{*}(\frac{\pi_{\theta}(x)}{p(x)})-\left(f^{*}(\frac{\pi_{\theta}(x)}{p(x)})-\frac{\pi_{\theta}(x)}{p(x)}f^{*'}(\frac{\pi_{\theta}(x)}{p(x)})\right)(\frac{p(x)}{\pi_{\theta}(x)})\right]\\&\quad+f^{'}(\infty)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)>0,p(x)\ge0\}}\nabla_{\theta}\pi_{\theta}(x)f^{*'}(\frac{\pi_{\theta}(x)}{p(x)})+f^{'}(\infty)\nabla_{\theta}p(\pi_{\theta}=0)\\
 & =\sum_{\{x:\pi_{\theta}(x)>0,p(x)\ge0\}}\pi_{\theta}(x)f^{*'}(\frac{\pi_{\theta}(x)}{p(x)})\nabla_{\theta}\log\pi_{\theta}(x)+\nabla_{\theta}\sum_{\{x:\pi_{\theta}(x)=0,p(x)>0\}}f^{'}(\infty)p(x)
\end{align*}
For the third equation we use the definition of perspective function
$f(t)=tf^{*}(\frac{1}{t})$ and its derivative, $f^{'}(t)=f^{*}(\frac{1}{t})+tf^{*'}(\frac{1}{t})(-\frac{1}{t^{2}})=f^{*}(\frac{1}{t})-\frac{1}{t}f^{*'}(\frac{1}{t})$.
For the last step, as aforementioned, with either condition (i) stating that the support of $p$ is contained in the support of $\pi_{\theta}$ for all $\theta \in \Theta$, or (ii) that the support of $\pi_{\theta}$ does not depend on $\theta$, the last term goes to zero, thus completing the proof.
\end{proof}

\begin{thm*}[Baseline based on $f$-divergence property]
For $f$-divergence $D_{f}(\pi_{\theta}||p)$ with any generator $f$,
there exists a generator $g$ with the same divergence $D_{f}(\pi_{\theta}||p)=D_{g}(\pi_{\theta}||p)$ such that
\begin{align*}
\nabla_{\theta}D_{g}(\pi_{\theta}||p) & =E_{x\sim\pi_{\theta}}\left[\left(f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)-b\right)\nabla_{\theta}\log\pi_{\theta}(x)\right]\\
 & =\nabla_{\theta}D_{f}(\pi_{\theta}||p)
\end{align*}
\end{thm*}

\begin{proof}
Recall that %the facts of $f$-divergence that 
$D_{f}(\pi_{\theta}||p)=D_{g}(\pi_{\theta}||p)$
%if and only if exists $b\in\mathbb{R}$ such that 
\ptmdI{when}
$g(x)=f(x)-b(x-1)$, for $b\in\mathbb{R}$ %,$ with arbitrary $b\in\mathbb{R}$.
Therefore, $\nabla_{\theta}D_{f}(\pi_{\theta}||p)=\nabla_{\theta}D_{g}(\pi_{\theta}||p)$
with $g^{'}\left(\frac{\pi_\theta(x)}{p(x)}\right)=f^{'}\left(\frac{\pi_\theta(x)}{p(x)}\right)-b$ 
% Recall the facts of $f$-divergence that $D_{f}=D_{g}$ if and only
% if $g(x)=f(x)-b(x-1),$ with arbitrary $b\in\mathbb{R}$.
% {\footnotesize{}\begin{align*}
% \nabla_{\theta}D_{g}(\pi_{\theta},p) & =E_{x\sim\pi_{\theta}}\left[g^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)\nabla_{\theta}\log\pi_{\theta}(x)\right]\\
%  & =E_{x\sim\pi_{\theta}}\left[\left(f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)-b\right)\nabla_{\theta}\log\pi_{\theta}(x)\right]\\
%  & =E_{x\sim\pi_{\theta}}\left[f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)\nabla_{\theta}\log\pi_{\theta}(x)\right]\\& \quad -bE_{x\sim\pi_{\theta}}\left[\nabla_{\theta}\log\pi_{\theta}(x)\right]\\
%  % & =E_{x\sim\pi_{\theta}}\left[f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)\nabla_{\theta}\log\pi_{\theta}(x)\right]\\&\quad -b\sum_{\forall x}\left[\nabla_{\theta}\pi_{\theta}(x)\right]\\
%  & =E_{x\sim\pi_{\theta}}\left[\left(f^{'}\left(\frac{\pi_{\theta}(x)}{p(x)}\right)\right)\nabla_{\theta}\log\pi_{\theta}(x)\right]\\
%  & =\nabla_{\theta}D_{f}(\pi_{\theta},p)
% \end{align*}}
\end{proof}



\begin{algorithm}[tb]
   \caption{$f$-DPG}
   \label{alg:f_dgp}
\begin{algorithmic}
   \STATE {\bfseries Input:}  unnormalized target distribution $P(\cdot)$, initial model $a(\cdot)$, $D_f$ generator $f(\cdot)$
   % \FOR{$i=1$ {\bfseries to} $m-1$}
   \STATE {\bfseries Initialize:} $\pit(\cdot) \gets a(\cdot)$, $Z \gets 0$, $N \gets 0$
   \FOR{each iteration do}
   \FOR{each episode do}
   \STATE sample $x$ from $\pit(\cdot)$
   \STATE $N \gets N+1$
   %\STATE $Z \gets Z+\frac{P(x)/\pit(x)-Z}{N}$
   \STATE $Z \gets Z+\frac{(P(x)/\pit(x))-Z}{N}$
   \qquad \COMMENT{Estimate $Z$ with historical samples}
   \STATE $p(\cdot) \gets P(\cdot)/Z$
   \STATE $\theta \gets \theta + \alpha^{(\theta)}f^{'}\left(\frac{\pit(x)}{p(x)}\right)\nabt\log\pit$
   \ENDFOR
   \ENDFOR
   \STATE {\bfseries Output:}  $\pit$
\end{algorithmic}
\end{algorithm}

